Multimodal Learning with Transformers: A Survey

Transformer is a promising neural network learner, and has achieved great success in various machine learning tasks. Thanks to the recent prevalence of multimodal applications and big data, Transformer-based multimodal learning has become a hot topic in AI research. This paper presents a comprehensive survey of Transformer techniques oriented at multimodal data. The main contents of this survey include: (1) a background of multimodal learning, Transformer ecosystem, and the multimodal big data era, (2) a theoretical review of Vanilla Transformer, Vision Transformer, and multimodal Transformers, from a geometrically topological perspective, (3) a review of multimodal Transformer applications, via two important paradigms, i.e., for multimodal pretraining and for specific multimodal tasks, (4) a summary of the common challenges and designs shared by the multimodal Transformer models and applications, and (5) a discussion of open problems and potential research directions for the community.

==> tables/VLP-model-comparison.tex <==
\begin{table*}[!h]
\caption{ VLP model comparison. region-of-interest (RoI),
The main difference lies in the composition of the input.
VL-BERT joint training for BERT and Faster RCNN, global feature END...... \magenta{``They assume the visual representations to be fixed and and given by supervised pre-trained visual encoders''}\cite{sun2019learning}.
new column: features (special design), insights.
}
\label{table:vlp-model-comparison}
\begin{center}
\resizebox{\textwidth}{!}{
%\color{magenta}
\begin{tabular}{ l | l | c | c | c | c}
\hline
model & inputs \red{details} & architecture & pre-train tasks & pre-train dataset & downstream task  \\
\hline
\hline
VideoBERT \cite{sun2019videobert} & video + sentence & single stream & & &  \\
ViLBERT \cite{lu2019vilbert} & image + sentence & two stream & & &  \\
LXMERT \cite{tan2019lxmert} & image + sentence & hybrid two 2 one & & & VQA and GQA  \\
VisualBERT \cite{li2019visualbert} & image + sentence & one stream & 2 & 4 &  \\
VL-BERT \cite{su2019vl} & image + sentence & one stream & & &  \\


% conditional masking
UNITER \cite{chen2020uniter} & one-stream & & & &  \\


% CBT is the first to demonstrate the effectiveness of BERT-style pre-training in a fully self-supervised way for video.
CBT \cite{sun2019learning} & video + sentence & & & &  \\



% similar to VisualBERT, special design is on its input.
Unicoder-VL \cite{li2020unicoder} & image + sentence & one-stream & & &  \\



B2T2 \cite{alberti2019fusion} & & & & &  \\



% unified
VLP \cite{zhou2020unified} & image + sentence & & & &  \\




% based on ViLBERT, multi-tasks, multi-datasets, special design is on input.
% ''In this work, we develop a multi-task model for discriminative vision-and-language tasks based on the recently proposed ViLBERT [27] model.''
12-in-1 \cite{lu202012} & & & & &  \\



% use detected image tags to further enhance pre-training
Oscar \cite{li2020oscar} & & & & &  \\







%ImageBERT \cite{} & & & & &  \\









% Pixel-BERT
Pixel-BERT \cite{huang2020pixel} & & & & &  \\







ActBERT \cite{zhu2020actbert} & video+text & & & &  \\




% multi-task, multi-stage, one-stream,
ImageBERT \cite{qi2020imagebert} & image+text & & & &  \\



% HERO, 2020, citation 90+, \cite{li2020hero}
HERO \cite{li2020hero} & video+text & & & &  \\





% However, most of the existing multimodal models are pre-trained for understanding tasks, leading to a pretrainfinetune discrepancy for generation tasks. This paper proposes UniVL: a Unified Video and Language pre-training model for both multimodal understanding and generation.
% It comprises four components, including two singlemodal encoders, a cross encoder, and a decoder with the Transformer backbone.
UniVL \cite{luo2020univl} & video+text & & & &  \\

& & & & &  \\

& & & & &  \\

& & & & &  \\

& & & & &  \\
\hline
\end{tabular}
}
\end{center}

\end{table*}





==> tables/architectures.tex <==
\begin{table}[!h]
\caption{ architectures.  combine figure \ref{fig:ViLT-figure2}, Common multimodal pretraining models fail for instance-level tasks \cite{zhan2021product1m}
}
\label{table:architectures}
\begin{center}
\resizebox{0.5\textwidth}{!}{
%\color{magenta}
\begin{tabular}{ l | l}
\hline
multimodal architecture & representative models \\
\hline
\hline
single-stream &  Uniter \cite{chen2020uniter}, Visualbert \cite{li2019visualbert},  Vl-bert \cite{su2019vl}  \\
\hline
two-stream &  Vl-bert \cite{su2019vl}, Lxmert \cite{tan2019lxmert},     \\
\hline
dual-stream &      \\
\hline
\end{tabular}
}
\end{center}

\end{table}

==> tables/models.tex <==

Pre-train task:

Pre-train Datasets

input
text encoding,
image/video encoding,



fusion

tokens:

mathematic formulation.



output




complexity

parameters

Downstream Tasks and performance evaluation

advantage

disadvantage

Hardware:

==> tables/vlp-pretraining-end-to-end-vs-two-stage.tex <==
\begin{table}[!h]
\caption{ architectures.  Common multimodal pretraining models fail for instance-level tasks \cite{zhan2021product1m}
}
\label{table:architectures}
\begin{center}
\resizebox{0.5\textwidth}{!}{
%\color{magenta}
\begin{tabular}{ l | l}
\hline
multimodal architecture & representative models \\
\hline
\hline
single-stream &  Uniter \cite{chen2020uniter}, Visualbert \cite{li2019visualbert},  Vl-bert \cite{su2019vl}  \\
\hline
two-stream &  Vl-bert \cite{su2019vl}, Lxmert \cite{tan2019lxmert},     \\
\hline
dual-stream &      \\
\hline
\end{tabular}
}
\end{center}

\end{table}

==> tex/ACL2021.tex <==





% UNIMO: Towards Unified-Modal Understanding and Generation via
% Cross-Modal Contrastive Learning \cite{li2020unimo}


Control Image Captioning Spatially and Temporally \cite{yan2021control}

VisualSparta: An Embarrassingly Simple Approach to Large-scale Text-to-Image Search with Weighted Bag-of-words \cite{lu2021visualsparta}

% PhotoChat: A Human-Human Dialogue Dataset with Photo Sharing
% Behavior for Joint Image-Text Modeling \cite{zang2021photochat}

% The GCM is a cross attention
Hierarchical Context-aware Network for Dense Video Event Captioning \cite{ji2021hierarchical}


% Multimodal Multihead Attention Interaction (MMAI) module    0 citation.
% Multimodal Sentiment Detection Based on Multi-channel
% Graph Neural Networks \cite{yang2021multimodal}


% Self-Supervised Multimodal Opinion Summarization \cite{im2021self}

Learning Relation Alignment for Calibrated Cross-modal Retrieval \cite{ren2021learningrelation}

KM-BART: Knowledge Enhanced Multimodal BART for Visual
Commonsense Generation \cite{xing2021km}


Multi-stage Pre-training over Simplified Multimodal Pre-training Models \cite{liu2021multi}


Missing Modality Imagination Network for Emotion Recognition with
Uncertain Missing Modalities \cite{zhao2021missing}

% 
Learning Language and Multimodal Privacy-Preserving Markers
of Mood from Mobile Data \cite{liang2021learning}


CTFN: Hierarchical Learning for Multimodal Sentiment Analysis Using
Coupled-Translation Fusion Network \cite{tang2021ctfn}


Cross-modal Memory Networks for Radiology Report Generation \cite{chen2021cross}


Multi-perspective Coherent Reasoning for Helpfulness Prediction of
Multimodal Reviews \cite{liu2021multiperspective}


% E2E-VLP: End-to-End Vision-Language Pre-training Enhanced by Visual
% Learning \cite{xu2021e2e} 11cit,

% ?
Edited Media Understanding Frames: Reasoning About the
Intents and Implications of Visual Disinformation \cite{da2021edited}


Check It Again: Progressive Visual Question Answering
via Visual Entailment \cite{si2021check}

% use
Mind Your Outliers! Investigating the Negative Impact of Outliers on
Active Learning for Visual Question Answering \cite{karamcheti2021mind}


Good for Misconceived Reasons: An Empirical Revisiting on the Need for
Visual Context in Multimodal Machine Translation \cite{wu2021good}


Maria: A Visual Experience Powered Conversational Agent \cite{liang2021maria}

==> tex/CVPR2020.tex <==



Multimodal Categorization of Crisis Events in Social Media \cite{abavisani2020multimodal}

% Sign Language Transformers:
% Joint End-to-end Sign Language Recognition and Translation \cite{camgoz2020sign}

% representative
% \red{Image Search with Text Feedback by Visiolinguistic Attention Learning} \cite{chen2020image}

% Meshed-Memory Transformer for Image Captioning \cite{cornia2020meshed}


% % RGB + optical flow,
% Actor-Transformers for Group Activity Recognition \cite{gavrilyuk2020actor}, 40+cit,

Normalized and Geometry-Aware Self-Attention Network
for Image Captioning \cite{guo2020normalized}, 50+cit,


% Towards Learning a Generic Agent for
% Vision-and-Language Navigation via Pre-training \cite{hao2020towards}, 


Iterative Answer Prediction with Pointer-Augmented
Multimodal Transformers for TextVQA \cite{hu2020iterative}, 60+cit,


Modality Shifting Attention Network for Multi-modal Video Question Answering \cite{kim2020modality}

Context-Aware Group Captioning via Self-Attention and Contrastive Features \cite{li2020context}

% GPS-Net: Graph Property Sensing Network for Scene Graph Generation \cite{lin2020gps}, 50+cit,


% Spatio-Temporal Graph for Video Captioning with Knowledge Distillation \cite{pan2020spatio},  80+cit,


% X-Linear Attention Networks for Image Captioning \cite{pan2020x}, 150+cit,


Video Object Grounding using Semantic Roles in Language Description \cite{sadhu2020video}, 

Transform and Tell: Entity-Aware News Image Captioning \cite{tran2020transform}


Multi-Modality Cross Attention Network for Image and Sentence Matching \cite{wei2020multi}

Towards Accurate Scene Text Recognition with Semantic Reasoning Networks \cite{yu2020towards}, 70+cita,

% no transformer
% Object Relational Graph with Teacher-Recommended Learning
% for Video Captioning  \cite{zhang2020object}, 90+cita,


% ActBERT: Learning Global-Local Video-Text Representations \cite{zhu2020actbert}, 100+cit.

What makes training multi-modal classification networks hard? \cite{wang2020makes}




==> tex/CVPR2021.tex <==
% Artemis: Affective language for visual art \cite{achlioptas2021artemis} \\

% Conceptual 12M (CC12M), a dataset with 12 million image-text pairs specifically meant to be used for visionand-language pre-training~\cite{changpinyo2021conceptual} \\

Human-like Controllable Image Captioning with Verb-specific Semantic Roles \cite{chen2021human}, Controllable Image Captioning (CIC), 

% Scene Text Telescope: Text-Focused Scene Image Super-Resolution \cite{chen2021scene}, , \\  not multimodal

% Semantic Audio-Visual Navigation \cite{chen2021semantic} \\


% Topological Planning with Transformers for Vision-and-Language Navigation \cite{chen2021topological} \\

% Sketch, Ground, and Refine: Top-Down Dense Video Captioning \cite{deng2021sketch} 

% Taming Transformers for High-Resolution Image Synthesis \cite{esser2021taming} \\

Read Like Humans: Autonomous, Bidirectional and Iterative Language Modeling for Scene Text Recognition \cite{fang2021read} 

% ARCH, a multiple instance captioning computational pathology dataset, CVPR 2021, Multiple Instance Captioning: Learning Representations from Histopathology Textbooks and Articles \cite{gamper2021multiple} \\

% VLNoeBERT: A Recurrent Vision-and-Language BERT for Navigation \cite{hong2021vln} \\

% Seeing Out of tHe bOx: End-to-End Pre-training for Vision-Language Representation Learning \cite{huang2021seeing} , 36cit,

% How Transferable are Reasoning Patterns in VQA? \cite{kervadec2021transferable} \\

% ClipBERT, Less is More: CLIPBERT for Video-and-Language Learning via Sparse Sampling \cite{lei2021less},

% VX2TEXT: End-to-End Learning of Video-Based Text Generation From Multimodal Inputs \cite{lin2021vx2text} \\

Adaptive Cross-Modal Prototypes for Cross-Domain Visual-Language Retrieval \cite{liu2021adaptive} 

% Traffic: Multimodal Motion Prediction with Stacked Transformers \cite{liu2021multimodal}    \\ 

% Progressive Modality Reinforcement for Human Multimodal Emotion Recognition from Unaligned Multimodal Sequences \cite{lv2021progressive}   \\

% KRISP: Integrating Implicit and Symbolic Knowledge for Open-Domain Knowledge-Based VQA \cite{marino2021krisp} \\


% https://zhuanlan.zhihu.com/p/396505571
% Thinking Fast and Slow: Efficient Text-to-Visual Retrieval with Transformers \cite{miech2021thinking}   

% M3P: Learning Universal Representations via Multitask Multilingual Multimodal Pre-training \cite{ni2021m3p} 

% Multi-Modal Fusion Transformer for End-to-End Autonomous Driving \cite{prakash2021multi} \\


% Learning from the Master: Distilling Cross-modal Advanced Knowledge for Lip Reading \cite{ren2021learning} \\


% Revamping Cross-Modal Recipe Retrieval with Hierarchical Transformers and Self-supervised Learning \cite{salvador2021revamping}   \\

Towards Diverse Paragraph Captioning for Untrimmed Videos \cite{song2021towards} 

% Read and Attend: Temporal Localisation in Sign Language Videos \cite{varol2021read}, 7cit, \\

Self-attention based Text Knowledge Mining for Text Detection \cite{wan2021self} 

Improving OCR-based Image Captioning by Incorporating Geometrical Relationship \cite{wang2021improving}    

% T2VLAD: Global-Local Sequence Alignment for Text-Video Retrieval \cite{wang2021t2vlad}   \\
 
Separating Skills and Concepts for Novel Visual Question Answering \cite{whitehead2021separating}  

% Fashion IQ: A New Dataset Towards Retrieving Images by Natural Language Feedback \cite{wu2021fashion}    \\

NExT-QA: Next Phase of Question-Answering to Explaining Temporal Actions \cite{xiao2021next}  

% Towards Accurate Text-based Image Captioning with Content Diversity Exploration
%\cite{xu2021towards}    \\

Primitive Representation Learning for Scene Text Recognition \cite{yan2021primitive}   

% Causal Attention for Vision-Language Tasks \cite{yang2021causal}   \\

% LayoutTransformer: Scene Layout Generation with Conceptual and Spatial Diversity \cite{yang2021layouttransformer}    \\

TAP: Text-Aware Pre-training for Text-VQA and Text-Caption \cite{yang2021tap} 

Multimodal Contrastive Training for Visual Representation Learning \cite{yuan2021multimodal}  

% Open-Vocabulary Object Detection Using Captions \cite{zareian2021open}   \\

% Domain-robust VQA with diverse datasets and methods but no target labels \cite{zhang2021domain} \\

% Multi-stage Aggregated Transformer Network for Temporal Language Localization in Videos  \cite{zhang2021multi}       \\

RSTNet: Captioning with Adaptive Attention on Visual and Non-Visual Words \cite{zhang2021rstnet}    

% VinVL: Revisiting Visual Representations in Vision-Language Models \cite{zhang2021vinvl} \\

% Improving Sign Language Translation with Monolingual Data by Sign Back-Translation \cite{zhou2021improving}  \\

% UC2: Universal Cross-lingual Cross-modal Vision-and-Language Pre-training \cite{zhou2021uc2} 15cit,   

% Kaleido-BERT: Vision-Language Pre-training on Fashion Domain \cite{zhuge2021kaleido}  

Cross-modal contrastive learning for text-to-image generation \cite{zhang2021cross}

==> tex/CVPR2022.tex <==






% Vision-Language Pre-Training with Triple Contrastive Learning \cite{yang2022vision}
%https://arxiv.org/pdf/2202.10401.pdf
%https://zhuanlan.zhihu.com/p/477300430

==> tex/ICASSP2021.tex <==


% Q K V
% Learning contextual tag embeddings for cross-modal alignment of audio and tags \cite{favory2021learning}


% Vset: A Multimodal Transformer for Visual Speech Enhancement \cite{ramesh2021vset}







Image-Assisted Transformer in Zero-Resource Multi-Modal Translation \cite{huang2021image}

==> tex/ICCV2019.tex <==









% 3D Scene Reconstruction with Multi-layer Depth and Epipolar Transformers \cite{shin20193d}

==> tex/ICCV2021.tex <==
% -----------------------------------------------------
%
%                          ICCV2021
%
%-------------------------------------------------------



% From General to Specific: Informative Scene Graph Generation via Balance Adjustment \cite{guo2021general}

% Target Adaptive Context Aggregation for Video Scene Graph Generation \cite{teng2021target}

% AI Choreographer: Music Conditioned 3D Dance Generation with AIST++ \cite{li2021ai}

% not transformer paper.
% Adaptive Hierarchical Graph Reasoning with Semantic Coherence for
% Video-and-Language Inference \cite{li2021adaptive}

% Learning to Generate Scene Graph from Natural Language Supervision \cite{zhong2021learning}

% Aligning Subtitles in Sign Language Videos \cite{bull2021aligning}


Zero-shot Natural Language Video Localization \cite{nam2021zero}


Synthesis of Compositional Animations from Textual Descriptions \cite{ghosh2021synthesis}

Explain Me the Painting: Multi-Topic Knowledgeable Art Description Generation \cite{bai2021explain}

Describing and Localizing Multiple Changes with Transformers \cite{qiu2021describing}


% Contrast and Classify: Training Robust VQA Models \cite{kant2021contrast}



Weakly Supervised Relative Spatial Reasoning for Visual Question Answering \cite{banerjee2021weakly}


% Pano-AVQA: Grounded Audio-Visual Question Answering on 360 Videos \cite{yun2021pano} 

% Just Ask: Learning to Answer Questions from Millions of Narrated Videos \cite{yang2021just}


On the hidden treasure of dialog in video question answering \cite{engin2021hidden}

Auto-Parsing Network for Image Captioning and Visual Question Answering \cite{yang2021auto}

% End-to-End Dense Video Captioning with Parallel Decoding \cite{wang2021end}


% Topic Scene Graph Generation by Attention Distillation from Caption \cite{wang2021topic}

% Cross-Sentence Temporal and Semantic Relations in Video Activity Localisation \cite{huang2021cross}


% Airbert: In-domain Pretraining for Vision-and-Language Navigation \cite{guhur2021airbert}


VLGrammar: Grounded Grammar Induction of Vision and Language \cite{hong2021vlgrammar} ???

% Vision-Language Navigation with Random Environmental Mixup \cite{liu2021vision}


% Image Retrieval on Real-life Images with Pre-trained
% Vision-and-Language Models \cite{liu2021image}

% The Road to Know-Where: An Object-and-Room Informed Sequential BERT
% for Indoor Vision-Language Navigation \cite{qi2021road}

% Unified Questioner Transformer for Descriptive Question Generation
% in Goal-Oriented Visual Dialogue \cite{matsumori2021unified}

TransVG: End-to-End Visual Grounding with Transformers \cite{deng2021transvg}


% LayoutTransformer: Layout Generation and Completion with Self-attention \cite{gupta2020layouttransformer}

% Visual Relationship Detection Using Part-and-Sum Transformers with Composite Queries 
% ? ? ?

Vision-Language Transformer and Query Generation for Referring
Segmentation \cite{ding2021vision}

% Episodic Transformer for Vision-and-Language Navigation \cite{pashevich2021episodic}

% Context-aware Scene Graph Generation with Seq2Seq Transformers \cite{lu2021context}


% LocalTrans: A Multiscale Local Transformer Network for Cross-Resolution Homography Estimation

% DocFormer: End-to-End Transformer for Document Understanding \cite{appalaraju2021docformer}


STVGBert: A Visual-linguistic Transformer based Framework
for Spatio-temporal Video Grounding \cite{su2021stvgbert}

TRAR: Routing the Attention Spans in Transformer for Visual Question Answering \cite{zhou2021trar}

% 3D Human Texture Estimation from a Single Image with Transformers \cite{xu20213d}

% 3DVG-Transformer: Relation Modeling for Visual Grounding on Point Clouds \cite{zhao20213dvg}

% The Right to Talk:
% An Audio-Visual Transformer Approach \cite{truong2021right} 2cit,

From Two to One: A New Scene Text Recognizer with
Visual Language Modeling Network \cite{wang2021two}


Who’s Waldo? Linking People Across Text and Images \cite{cui2021s}

StyleCLIP: Text-Driven Manipulation of StyleGAN Imagery \cite{patashnik2021styleclip}


HiT: Hierarchical Transformer with Momentum Contrast for Video-Text
Retrieval \cite{liu2021hit}

TACo: Token-aware Cascade Contrastive Learning for Video-Text Alignment \cite{yang2021taco}


DAE-GAN: Dynamic Aspect-aware GAN for Text-to-Image Synthesis \cite{ruan2021dae}

Beyond Question-Based Biases:
Assessing Multimodal Shortcut Learning in Visual Question Answering \cite{dancette2021beyond}


% COOKIE: Contrastive Cross-Modal Knowledge Sharing Pre-training
% for Vision-Language Representation \cite{wen2021cookie}


Attention is not Enough: Mitigating the Distribution Discrepancy in
Asynchronous Multimodal Sequence Fusion \cite{liang2021attention}


% Multimodal Co-Attention Transformer for Survival Prediction
% in Gigapixel Whole Slide Images \cite{chen2021multimodal}



Space-Time Crop \& Attend:
Improving Cross-modal Video Representation Learning \cite{patrick2021space}


Multi-Modal Multi-Action Video Recognition \cite{shi2021multi}

% Product1M: TowardsWeakly Supervised Instance-Level Product Retrieval
% via Cross-Modal Pretraining \cite{zhan2021product1m}

Generic Attention-model Explainability for Interpreting
Bi-Modal and Encoder-Decoder Transformers \cite{chefer2021generic}


Telling the What while Pointing to the Where:
Multimodal Queries for Image Retrieval \cite{changpinyo2021telling}

% TEACHTEXT: CrossModal Generalized Distillation for Text-Video Retrieval 
% To provide an extensive comparison we test our approach
% on seven video datasets that have been explored in recent
% works as benchmarks for the task of text-video retrieval:
% LSMDC [42], DiDeMo [1], MSVD [11], MSRVTT [55],
% ActivityNet [9], VaTeX [53] and QuerYD [36]. We follow
% the same experimental setup as prior works [12, 18, 28, 39].


MDETR - Modulated Detection for End-to-End Multi-Modal Understanding \cite{kamath2021mdetr}


CrossCLR: Cross-modal Contrastive Learning For Multi-modal Video Representations \cite{zolfaghari2021crossclr}


% UniT: Multimodal Multitask Learning with a Unified Transformer \cite{hu2021unit}




==> tex/ICLR2021.tex <==





% Adaspeech: Adaptive text to speech for custom voice \cite{chen2021adaspeech}, 17cit,   \\

ALFWorld: Aligning text and embodied environments 
for interactive learning \cite{shridhar2020alfworld}  

Answering complex open-domain questions with multi-hop dense retrieval\cite{xiong2020answering}  


%Dance Revolution: Long-Term Dance Generation with Music via Curriculum Learning \cite{huang2020dance} 

% Fastspeech 2: Fast and high-quality end-to-end text to speech \cite{ren2020fastspeech}, 190+ citations. \\


% Graphcodebert: Pre-training code representations with data flow \cite{guo2020graphcodebert}, 50+ citations. \\

% Language-agnostic representation learning of source code from structure and context \cite{zugner2021language} \\

% MultiModalQA: Complex Question Answering over Text, Tables and Images \cite{talmor2021multimodalqa} 

% Open question answering over tables and text \cite{chen2020open}

% Parameter efficient multimodal transformers for video representation learning \cite{lee2020parameter}

Support-set bottlenecks for video-text representation learning \cite{patrick2020support}

==> tex/ICML2021.tex <==
% Unifying Vision-and-Language Tasks via Text Generation \cite{cho2021unifying} 34 cit, \\

% Fused Acoustic and Text Encoding for Multimodal Bilingual Pretraining and Speech Translation \cite{zheng2021fused} \\

Grounding Language to Entities and Dynamics for Generalization in Reinforcement Learning \cite{wang2021grounding}  

PipeTransformer: Automated Elastic Pipelining for Distributed Training of Large-scale Models \cite{he2021pipetransformer}  

% Conditional Variational Autoencoder with Adversarial Learning for End-to-End Text-to-Speech \cite{kim2021conditional} \\

% EfficientTTS: An Efficient and High-Quality Text-to-Speech Architecture \cite{miao2021efficienttts} \\

% Meta-StyleSpeech : Multi-Speaker Adaptive Text-to-Speech Generation \cite{min2021meta}

% Grad-TTS: A Diffusion Probabilistic Model for Text-to-Speech \cite{popov2021grad}  \\

% Zero-Shot Text-to-Image Generation \cite{ramesh2021zero}, 220+ citations. 

% Perceiver: General Perception with Iterative Attention \cite{jaegle2021perceiver}, 65+cit,

==> tex/NeurIPS2020.tex <==




COOT: Cooperative Hierarchical Transformer for Video-Text Representation Learning \cite{ging2020coot}


% ? 
% Glow-TTS: A Generative Flow for Text-to-Speech via
% Monotonic Alignment Search \cite{kim2020glow} 60+ cit,


% Large-Scale Adversarial Training for
% Vision-and-Language Representation Learning \cite{gan2020large} 110+ cit,


% Learning Representations from Audio-Visual
% Spatial Alignment \cite{morgado2020learning}

==> tex/NeurIPS2021.tex <==
% Attention Bottlenecks for Multimodal Fusion \cite{nagrani2021attention} \\

% End-to-end Multi-modal Video Temporal Grounding \cite{chen2021end} \\

Evidential Softmax for Sparse Multimodal Distributions in Deep Generative Models \cite{chen2021evidential} 
% Explainable Semantic Space by Grounding Language to Vision with Cross-Modal Contrastive Learning \cite{zhang2021explainable} \\
% Exploring Cross-Video and Cross-Modality Signals for Weakly-Supervised Audio-Visual Video Parsing \cite{lin2021exploring} \\

% History Aware Multimodal Transformer for Vision-and-Language Navigation \cite{chen2021history} \\

% MERLOT: Multimodal Neural Script Knowledge Models \cite{zellers2021merlot} \\

% Multimodal and Multilingual Embeddings for Large-Scale Speech Mining \cite{duquenne2021multimodal} \\

Multimodal Few-Shot Learning with Frozen Language Models \cite{tsimpoukelli2021multimodal}  

% Probing Inter-modality: Visual Parsing with Self-Attention for Vision-Language Pre-training \cite{xue2021probing} , 6 cit,  \\

% UFC-BERT: Unifying Multi-Modal Controls for Conditional Image Synthesis \cite{zhang2021ufc}  \\

% VATT: Transformers for Multimodal Self-Supervised Learning from \red{Raw Video, Audio and Text}  \cite{akbari2021vatt}  

% Align before fuse: Vision and language representation learning with momentum distillation \cite{li2021align} 30cit,

ATISS: Autoregressive Transformers for Indoor Scene Synthesis \cite{paschalidou2021atiss} 

% CLIP-It! language-guided video summarization \cite{narasimhan2021clip}

% CogView: Mastering Text-to-Image Generation via Transformers \cite{ding2021cogview}


% Curriculum Learning for Vision-and-Language Navigation \cite{zhang2021curriculum}

% QVHighlights: Detecting Moments and Highlights in Videos via Natural Language Queries \cite{lei2021qvhighlights}

% Dynamic population-based meta-learning for multi-agent communication with natural language \cite{gupta2021dynamic}

% Explainable Semantic Space by Grounding Language to Vision with Cross-Modal Contrastive Learning \cite{zhang2021explainable}


Grounding Spatio-Temporal Language with Transformers \cite{karch2021grounding}

% Human-Adversarial Visual Question Answering \cite{sheng2021human}


% Introspective Distillation for Robust Question Answering \cite{niu2021introspective} 0cit,


Learning from Inside: Self-driven Siamese Sampling and Reasoning for Video Question Answering \cite{yu2021learning}


% Learning Knowledge Graph-based World Models of Textual Environments \cite{ammanabrolu2021learning}


% Long-short transformer: Efficient transformers for language and vision \cite{zhu2021long}


% PortaSpeech: Portable and High-Quality Generative Text-to-Speech \cite{ren2021portaspeech}


% Proto: Program-guided transformer for program-guided tasks \cite{zhao2021proto}


% Referring Transformer: A One-step Approach to Multi-task Visual Grounding \cite{li2021referring}


% Robust Visual Reasoning via Language Guided Neural Module Networks \cite{akula2021robust}


% SADGA: Structure-Aware Dual Graph Aggregation Network for Text-to-SQL \cite{cai2021sadga}


% SOAT: A Scene-and Object-Aware Transformer for Vision-and-Language Navigation \cite{moudgil2021soat}


% Speech-T: Transducer for Text to Speech and Beyond  \cite{chen2021speech} 

% Supervising the Transfer of Reasoning Patterns in VQA \cite{kervadec2021supervising}




VidLanKD: Improving Language Understanding via Video-Distilled Knowledge Transfer \cite{tang2021vidlankd}

==> tex/WACV2022.tex <==
Masking Modalities for Cross-modal Video Retrieval \cite{gabeur2022masking}

% Beyond Mono to Binaural: Generating Binaural Audio from Mono Audio with
% Depth and Cross Modal Attention \cite{parida2022beyond}

==> tex/arXiv2020.tex <==






Time: Text and image mutual-translation adversarial networks \cite{liu2020time}



% Interbert: Vision-and-language interaction for multi-modal pretraining \cite{lin2020interbert}




% OmniNet: A unified architecture for multi-modal
% multi-task learning \cite{pramanik2019omninet}

==> tex/arXiv2021.tex <==



% SGEITL: Scene Graph Enhanced Image-Text Learning for Visual Commonsense Reasoning \cite{wang2021sgeitl}


LMR-CBT: Learning Modality-fused Representations with CB-Transformer for Multimodal Emotion Recognition from Unaligned Multimodal Sequences \cite{fu2021lmr}


% MutualFormer: Multi-Modality Representation Learning via Mutual Transformer https://arxiv.org/pdf/2112.01177.pdf

% UFO: A UniFied TransfOrmer for Vision-Language Representation Learning \cite{wang2021ufo}


% Multimodal Transformer with Variable-length Memory for Vision-and-Language Navigation \cite{lin2021multimodal}

Egocentric Human Trajectory Forecasting with a Wearable Camera
and Multi-Modal Fusion \cite{qiu2021egocentric}


Cross-Modality Fusion Transformer for Multispectral Object Detection \cite{qingyun2021cross}


Visual Keyword Spotting with Attention \cite{prajwal2021visual}

% ?
% From Multimodal to Unimodal Attention in Transformers using Knowledge
% Distillation \cite{agarwal2021multimodal}

STREAMULT: STREAMING MULTIMODAL TRANSFORMER FOR HETEROGENEOUS
AND ARBITRARY LONG SEQUENTIAL DATA \cite{pellegrain2021streamult}

% Dual-Level Collaborative Transformer for Image Captioning \cite{luo2021dual}

% not a multimodal paper, but a special architecture can be used for multimodal inputs.
% Mobile-Former: Bridging MobileNet and Transformer \cite{chen2021mobile}



% Cpt: Colorful prompt tuning for pre-trained vision-language models \cite{yao2021cpt} 4cit,


% SLIP: Self-supervision meets Language-Image Pre-training \cite{mu2021slip} ???



% Scheduled Sampling in Vision-Language Pretraining with Decoupled Encoder-Decoder Network \cite{li2021scheduled}


% Simvlm: Simple visual language model pretraining with weak supervision \cite{wang2021simvlm}




% GilBERT: Generative Vision-Language Pre-Training for Image-Text Retrieval \cite{hong2021gilbert} 2cit,

==> tex/arXiv2022.tex <==

% Learning Audio-Visual Speech Representation by Masked Multimodal Cluster Prediction \cite{shi2022learning}




%  https://arxiv.org/pdf/2201.05078.pdf
% CLIP-Event: Connecting Text and Images with Event Structures \cite{li2022clip}


%https://arxiv.org/pdf/2201.05729.pdf
% CLIP-TD: CLIP Targeted Distillation for Vision-Language Tasks \cite{wang2022clip}


% Omnivore: A Single Model for Many Visual Modalities \cite{girdhar2022omnivore}
% https://arxiv.org/abs/2201.08377


% Transformers in Medical Imaging: A Survey \cite{shamshad2022transformers}
% % https://arxiv.org/pdf/2201.09873.pdf


FIGARO: Generating Symbolic Music with Fine-Grained Artistic Control \cite{von2022figaro}
%https://arxiv.org/abs/2201.10936


Natural Language Descriptions of Deep Visual Features \cite{hernandez2022natural}
%https://openreview.net/pdf?id=NudBMY-tzDr   ICLR 2022


% OpenAI发布CLIP模型快一年了，盘点那些CLIP相关让人印象深刻的工作


% BLIP: Bootstrapping Language-Image Pre-training for Unified Vision-Language Understanding and Generation \cite{li2022blip}
% https://arxiv.org/abs/2201.12086


DEEP LEARNING APPROACHES ON IMAGE CAPTIONING: A
REVIEW \cite{ghandi2022deep}
% https://arxiv.org/pdf/2201.12944.pdf 


% Unifying Architectures, Tasks, and Modalities Through a Simple Sequence-to-Sequence Learning Framework
% https://arxiv.org/abs/2202.03052




% cross-modal generation
% CLIPasso: Semantically-Aware Object Sketching \cite{vinker2022clipasso}


% https://mp.weixin.qq.com/s/AClFYBovJA2xPQ3C-Q4Apg
Image Difference Captioning with Pre-training and Contrastive Learning \cite{yao2022image}


% https://arxiv.org/pdf/2202.07247.pdf
% CommerceMM: Large-Scale Commerce MultiModal
% Representation Learning with Omni Retrieval \cite{yu2022commercemm}

% https://arxiv.org/pdf/2202.08360v1.pdf
% Meta AI Research
% Vision Models Are More Robust And Fair When Pretrained On Uncurated Images Without Supervision \cite{goyal2022vision}


ViNTER: Image Narrative Generation with Emotion-Arc-Aware Transformer \cite{uehara2022vinter}


% Survey on Large Scale Neural Network Training
% J Gusak, D Cherniuk, A Shilova, A Katrutsa, D Bershatsky, X Zhao, L Eyraud-Dubois, O Shlyazhko, D Dimitrov, I Oseledets, O Beaumont
% [Skolkovo Institute of Science and Technology & University of Lille & University of Bordeaux & Sber AI]


%Visual Attention Network
% M Guo, C Lu, Z Liu, M Cheng, S Hu
% [Tsinghua University & Nankai University]



Self-Supervised Vision Transformers Learn
Visual Concepts in Histopathology
% https://arxiv.org/pdf/2203.00585.pdf





% % https://arxiv.org/pdf/2202.07125.pdf
% Transformers in Time Series: A Survey \cite{}



% not transformer
% Freeform Body Motion Generation from Speech \cite{}


Mind the Gap: Understanding the Modality Gap in Multi-modal Contrastive Representation Learning \cite{}


% DiT: Self-supervised Pre-training for Document Image Transformer \cite{li2022dit}

==> tex/audio-and-speech.tex <==
% Speech-to-SQL: Towards Speech-driven SQL Query Generation From Natural Language Question \cite{song2022speech}
% https://arxiv.org/pdf/2201.01209.pdf


% TriBERT: Full-body Human-centric Audio-visual Representation Learning for Visual Sound Separation \cite{rahman2021tribert}
% https://proceedings.neurips.cc/paper/2021/file/51200d29d1fc15f5a71c1dab4bb54f7c-Paper.pdf


% FaceFormer: Speech-Driven 3D Facial Animation with Transformers \cite{fan2021faceformer}

==> tex/cross-attention.tex <==



CrossViT: Cross-Attention Multi-Scale Vision Transformer for Image
Classification \cite{chen2021crossvit}, 70+citations.

==> tex/crossmodal-attention-blocks.tex <==











Attention is not Enough: Mitigating the Distribution Discrepancy in
Asynchronous Multimodal Sequence Fusion \cite{liang2021attention}




Multimodal Co-Attention Transformer for Survival Prediction
in Gigapixel Whole Slide Images \cite{chen2021multimodal}

==> tex/figures.tex <==





\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/Masked-Acoustic-Modeling.png}
	\caption{MAM: Masked Acoustic Modeling for End-to-End Speech-to-Text Translation}
	%\vspace{-0.6cm}
	\label{fig:Masked-Acoustic-Modeling}
\end{figure}


% ------------------------------


\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/ViLT-figure2.png}
	\caption{ViLT: Vision-and-Language Transformer
Without Convolution or Region Supervision}
	%\vspace{-0.6cm}
	\label{fig:ViLT-figure2}
\end{figure}




\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/Multiview-Transformers-for-Video-Recognition.png}
	\caption{Multiview-Transformers-for-Video-Recognition}
	%\vspace{-0.6cm}
	\label{fig:Multiview-Transformers-for-Video-Recognition}
\end{figure}




\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/VLP-methods.png}
	\caption{GilBERT: Generative Vision-Language Pre-Training for
Image-Text Retrieval
}
	%\vspace{-0.6cm}
	\label{fig:VLP-methods}
\end{figure}



\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/Tri-modal-Co-attention.png}
	\caption{TriBERT: Full-body Human-centric Audio-visual
Representation Learning for Visual Sound Separation}
	%\vspace{-0.6cm}
	\label{fig:Tri-modal-Co-attention}
\end{figure}





\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/X-Linear Attention.png}
	\caption{X-Linear Attention Networks for Image Captioning}
	%\vspace{-0.6cm}
	\label{fig:X-Linear-Attention}
\end{figure}





\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/UniVL-2.png}
	\caption{}
	%\vspace{-0.6cm}
	\label{fig:UniVL-2}
\end{figure}



\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{./figures/UniVL.png}
	\caption{}
	%\vspace{-0.6cm}
	\label{fig:UniVL}
\end{figure}






\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/EnTangled-Attention-ETA.png}
	\caption{}
	%\vspace{-0.6cm}
	\label{fig:EnTangled-Attention-ETA}
\end{figure}






\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/tangled-transformer.png}
	\caption{ActBERT: Learning Global-Local Video-Text Representations, CVPR 2020}
	%\vspace{-0.6cm}
	\label{fig:tangled-transformer}
\end{figure}

\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/two-stream-decoupled.png}
	\caption{Scheduled Sampling in Vision-Language Pretraining
with Decoupled Encoder-Decoder Network}
	%\vspace{-0.6cm}
	\label{fig:two-stream-decoupled}
\end{figure}







\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/three-architectures.png}
	\caption{HiT: Hierarchical Transformer with Momentum Contrast for Video-Text Retrieval, ICCV 2021}
	%\vspace{-0.6cm}
	\label{fig:three-architectures}
\end{figure}

\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/multi-self-supervised.png}
	\caption{Sound and Visual Representation Learning with Multiple Pretraining Tasks }
	%\vspace{-0.6cm}
	\label{fig:multi-self-supervised}
\end{figure}



\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/self-attention-and-co-attention.png}
	\caption{Generic Attention-model Explainability for Interpreting
Bi-Modal and Encoder-Decoder Transformers, ICCV 2021}
	%\vspace{-0.6cm}
	\label{fig:self-attention-and-co-attention}
\end{figure}


\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/MMAI.png}
	\caption{Multimodal Sentiment Detection Based on Multi-channel Graph Neural Networks, ACL 2021}
	%\vspace{-0.6cm}
	\label{fig:MMAI}
\end{figure}


\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/tasks.png}
	\caption{Simvlm: Simple visual language model pretraining with weak supervision}
	%\vspace{-0.6cm}
	\label{fig:tasks}
\end{figure}



\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/Multiview-Transformers-for-Video-Recognition.png}
	\caption{Multiview Transformers for Video Recognition, arXiv 2022}
	%\vspace{-0.6cm}
	\label{fig:Multiview-Transformers-for-Video-Recognition}
\end{figure}




\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/co-attention.png}
	\caption{Improving Fake News Detection by Using an Entity-enhanced
Framework to Fuse Diverse Multimodal Clues, ACM MM 2021}
	%\vspace{-0.6cm}
	\label{fig:co-attention}
\end{figure}



\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/Video-Transformers-A-Survey.png}
	\caption{Video-Transformers-A-Survey, arXiv 2022.}
	%\vspace{-0.6cm}
	\label{fig:Video-Transformers-A-Survey}
\end{figure}


\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/two-view-transformer.png}
	\caption{TVT: Two-View Transformer Network for Video Captioning}
	%\vspace{-0.6cm}
	\label{fig:two-view-transformer}
\end{figure}



\begin{figure}[!th]
	\centering	
	\includegraphics[width=\linewidth]{./figures/BimodalCrossAttentionLayer.png}
	\caption{Humor Knowledge Enriched Transformer for Understanding Multimodal Humor, AAAI 2021. \cite{}}
	%\vspace{-0.6cm}
	\label{fig:Bimodal-Cross-Attention-Layer}
\end{figure}


==> tex/healthcareAI.tex <==





% no transformer, multi-modal healthcare application.
% CheXstray: Real-time Multi-Modal Data Concordance for Drift Detection in Medical Imaging AI





% Multimodal Co-Attention Transformer for Survival Prediction in Gigapixel Whole Slide Images \cite{chen2021multimodal}

==> tex/multimodal-applications.tex <==

%--------------------------------------------------------
%
%                 multimodal applications
%
%--------------------------------------------------------



% \red{Multimodal Applications:} \\

% IMPORTANT --
% Open Table-and-Text Question Answering (OTT-QA) \cite{chen2020open}


% Navigation: \\
% Audio-Visual Navigation \cite{chen2021semantic} \\
% Vision-and-Language Navigation \cite{chen2021topological, hong2021vln} \\


% Multimodal Motion Prediction for traffic \cite{liu2021multimodal} \\

% Multimodal Emotion Recognition \cite{lv2021progressive}

% multimodal event representation \cite{zellers2021merlot} \\


% DEFINITION definition \magenta{``Visual Commonsense Reasoning (VCR)[8] requires the model can not only answer the commonsense question
% but also select a rationale to support the answer'' \cite{qi2020imagebert}}


% Vision2semantic understanding: \\
% Image captioning,  \\
% Text-based image caption \cite{xu2021towards} 
% OCR-based Image Captioning  \\
% video cationing, Dense Video Captioning (DVC) \\
% VQA , video QA VideoQA\cite{le2021dvd}, Videogrounded Dialogues \cite{le2021dvd}, \\
% but transformer methods handle real linguistic and some visual shifts better due to pretraining. \cite{zhang2021domain}


% not transformer
% Human-Adversarial Visual Question Answering \cite{sheng2021human} 




% Video-Based Text Generation \cite{lin2021vx2text} 

% AI Choreographer: Music Conditioned 3D Dance Generation with AIST++ \cite{li2021ai}

% cross-modal generation: \\
% image Synthesis \\
% OCR, detect text from image \\
% Scene Layout Generation \cite{yang2021layouttransformer}  \\
% Sign Language Translation \cite{zhou2021improving}  \\
% Learning to Generate Scene Graph from Natural Language Supervision \cite{zhong2021learning} \\
% speech-to-SQL \cite{song2022speech} \\
% text-to-SQL \cite{cai2021sadga} \\


% cross-modal retrieval:\\
% Cross-Domain Visual-Language Retrieval \\
% Text-to-Visual Retrieval \\
%Text-Video Retrieval, text-to-video retrieval \cite{wang2021t2vlad},
% Multi-query Video Retrieval
% \cite{wang2022multi} 
% Cross-Modal Recipe Retrieval \cite{salvador2021revamping} \\
% Retrieving Images by Natural Language Feedback \cite{wu2021fashion} \\

%multimodal perception: 

% for Autonomous Driving \cite{prakash2021multi},
% %Audio-Visual Navigation \cite{chen2021semantic} \\
% Vision-and-Language Navigation \cite{chen2021topological, hong2021vln} \\
End-to-end Multi-modal Video Temporal Grounding \cite{chen2021end} 
% Audio-Visual Video Parsing \cite{lin2021exploring} \\
% Multimodal Event Representation \cite{zellers2021merlot} \\
% Parameter efficient multimodal transformers for video representation learning \cite{lee2020parameter}, 27cit, \\

Open-Vocabulary Object Detection Using Captions \cite{zareian2021open} 



Temporal Language Localization in Videos \cite{zhang2021multi}    

% Face, Body, Voice: Video Person-Clustering with Multiple Modalities \cite{brown2021face} \\

% Speech2Action: Cross-modal Supervision for Action Recognition \cite{nagrani2020speech2action}, a BERT based model \\


% Multimodal Bilingual Pretraining and Speech Translation \cite{zheng2021fused} \\

Language as Queries for Referring Video Object Segmentation \cite{wu2022language}  

% Text-to-speech \cite{%miao2021efficienttts, 
% min2021meta, popov2021grad} 

% zero-shot Text-to-Image Generation \cite{ramesh2021zero}

% CogView: Mastering Text-to-Image Generation via Transformers \cite{ding2021cogview}

% CLIP-Forge: Towards Zero-Shot Text-to-Shape Generation \cite{sanghi2021clip}\\

% semantics-controlled multi-modal shuffled Transformer reasoning,
% Dynamic Graph Representation Learning for Video Dialog via Multi-Modal Shuffled Transformers \cite{geng2021dynamic}    


% Grounding Language to Vision \cite{zhang2021explainable} 

% VATT: Transformers for Multimodal Self-Supervised Learning from \red{Raw Video, Audio and Text}  \cite{akbari2021vatt}  

% MultiModalQA: Complex Question Answering over 
% \red{Text, Tables and Images} \cite{talmor2021multimodalqa} 


% CLIP-It! language-guided video summarization \cite{narasimhan2021clip}


QVHighlights: Detecting Moments and Highlights in Videos via Natural Language Queries \cite{lei2021qvhighlights}

Dynamic population-based meta-learning for multi-agent communication with natural language \cite{gupta2021dynamic}


% GQA visual reasoning, ProTo: Program-Guided Transformer
% for Program-Guided Tasks, \cite{zhao2021proto}



Referring Transformer: A One-step Approach to Multi-task Visual Grounding \cite{li2021referring}


% Text-to-SQL \cite{cai2021sadga}

% Scene Graph Generation \cite{guo2021general} \\
% Target Adaptive Context Aggregation for Video Scene Graph Generation \cite{teng2021target}, 3cit,

% AI Choreographer: Music Conditioned 3D Dance Generation with AIST++ \cite{li2021ai}


% Learning to Generate Scene Graph from Natural Language Supervision \cite{zhong2021learning}


% Textual Description and Point Cloud \cite{zhao20213dvg}

% Speech2Action: Cross-modal Supervision for Action Recognition \cite{nagrani2020speech2action} \\


Self-Supervised Multimodal Opinion Summarization \cite{im2021self}

% LayoutLMv2: Multi-modal Pre-training for Visually-rich
% Document Understanding \cite{xu2020layoutlmv2}


PLOTCODER: Hierarchical Decoding for Synthesizing Visualization Code
in Programmatic Context \cite{chen2021plotcoder}

% text-to-SQL ?
% KaggleDBQA: Realistic Evaluation of Text-to-SQL Parsers. 
% Chase: A Large-Scale and Pragmatic Chinese Dataset for Cross-Database Context-Dependent Text-to-SQL. 



Multimodal Personality Recognition using Cross-Attention Transformer and Behaviour Encoding \cite{agrawal2021multimodal}


Learning Semantic-Aligned Feature Representation for Text-based Person Search \cite{li2021learning}

ITA: Image-Text Alignments for Multi-Modal Named Entity Recognition \cite{wang2021ita}

% two modalities: CT and MR
Dispensed Transformer Network for Unsupervised Domain Adaptation \cite{li2021dispensed}

Improving Fake News Detection by Using an Entity-enhanced Framework to Fuse Diverse Multimodal Clues \cite{qi2021improving}



% Humor Knowledge Enriched Transformer for Understanding Multimodal Humor \cite{hasan2021humor}

==> tex/multiview.tex <==


%https://arxiv.org/pdf/2201.04288.pdf
%Multiview Transformers for Video Recognition

==> tex/notes.tex <==
% GPT-2 \cite{radford2019language}, 
% GPT-3 \cite{brown2020language},
%DVD \cite{le2021dvd},
%PhotoChat \cite{zang2021photochat}.
% CNERTA \cite{sui2021large},
















% 为什么Transformer适合做多模态任务？

% https://www.zhihu.com/question/441073210

% 多模态：自动驾驶中的多模态学习
% https://zhuanlan.zhihu.com/p/328671301





% Reading list for research topics in Masked Image Modeling(MIM).
% https://github.com/ucasligang/awesome-MIM


% 量子启发的多模态融合模型
% https://mp.weixin.qq.com/s/VUIU8xF0x3WMLEG_q6imLw


% 从LXMERT到VLMO：多模态预训练模型的演变史
% https://mp.weixin.qq.com/s/dtEESJjGXaRNwEhV9EDPcw


% 万字综述！从21篇最新论文看多模态预训练模型研究进展
% https://mp.weixin.qq.com/s/gyGeFHV2jlgCQaGmWBKMVQ


% ACM MM 2021 | 面向多模态情绪识别的双流异质图递归神经网络
% https://mp.weixin.qq.com/s/uQhFLbb0zhXDsji4c4MkwQ


% 从多篇2021年顶会论文看多模态预训练模型最新研究进展
% https://mp.weixin.qq.com/s/eq4uxtt3QSFzCdkD5eyMVQ


% 中科院自动化所：最新视觉-语言预训练综述
% https://mp.weixin.qq.com/s/bpD4fNaK6GJlo7LWFOY3Rg
% https://arxiv.org/pdf/2202.09061.pdf









\keypoint{\red{some key points:}} \\

% (0) What is multimodal learning and why is it important \cite{baltruvsaitis2018multimodal}?

(1) Highlight CLIP open a new era of ``zero-shot'' and transfering classification/recognition as retrieval 

(2) ViT is a milestone. Pre-ViT era: faster-RCNN + transformer, Post-ViT era.

% (3) \red{Eddy: Transformer is suitable for multi-modal fusion. Why?}

(4) Peng: try to look for some mathematical papers.

(5) Louis-Philippe Morency (author of that PAMI survey) has a lot of multimodal papers, need to cite.


\keypoint{Key Questions to ask AZ:} \\
(1) How to define modality? \\
(2) Why is Transformer suitable for multimodal tasks? \\
(3) \\

%  A Survey on Vision Transformer
% https://mp.weixin.qq.com/s/tloHFx-ngO8h7Oi3m4rjrg

% A Survey on Vision Transformer
% https://mp.weixin.qq.com/s/J6mBIdT-sHQKd6zG0tAfKQ


Microsoft coco captions: Data collection and evaluation server \cite{chen2015microsoft}



% https://mp.weixin.qq.com/s/nOCyAIXgRHdcktXkgm_Kcw
% 单GPU每秒76帧，重叠对象也能完美分割，多模态Transformer用于视频分割效果惊艳
% https://arxiv.org/pdf/2111.14821.pdf
% CVPR 2022,




Visual question answering in the medical domain based on deep learning approaches: A comprehensive study

% Vision Transformer必读系列之图像分类综述：Attention-based
% https://mp.weixin.qq.com/s/84e4QBEsf6n0lCQfCSLnDg


3D CNN video,
I3D \cite{carreira2017quo},




% -------------------------------
KD-VLP: Improving End-to-End Vision-and-Language Pretraining with
Object Knowledge Distillation



Two-step Pretraining The two-step pretraining methods
firstly employ an off-the-shelf object detector to convert
an image into a set of object embeddings, and then feed
them into a Transformer jointly with text embeddings to
generate their multi-modal representations. Hence their visual feature networks are not optimized during both pretraining & finetuning stage. Most of these methods, such as
LXMERT (Tan and Bansal 2019),ViLBert (Lu et al. 2019),
VL-Bert (Su et al. 2020), Unicoder-VL (Li et al. 2020a) and
UNITER (Chen et al. 2020), adopt BERT-like objectives to
train their networks, which include Masked Language Modeling (MLM), Masked Vision Modeling (MVM) and ImageText Matching (ITM). In addition, VILLA (Gan et al. 2020)
develops an advanced adversarial pretraining and finetuning
strategy to improve generalization ability. OSCAR (Li et al.
2020b) and VINVL (Zhang et al. 2021) introduce object labels to bridge different modalities and revisit the importance
of visual features. Ernie-ViL (Yu et al. 2020) exploits structured knowledge in the text and constructs scene graph prediction tasks to learn joint representations. UNIMO (Li et al.
2021) proposes a unified model to leverage large-scale free
text corpus, image collections, and image-text pairs simultaneously through a contrastive learning task. Despite their
strong performances, those methods are limited by the object
detector and neglect visual cues outside of object regions,
often leading to mistakes in downstream tasks.
End-to-End (E2E) Pretraining The E2E pretraining approaches directly feed dense features on image grids from
a visual backbone network into a Transformer network
along with text tokens. As such, both the visual and Transformer networks are optimized jointly in an end-to-end manner in the pretraining & finetuning stage. Pixel-Bert and
SOHO (Huang et al. 2021, 2020) pioneer the use of the
E2E pretraining architecture and propose a novel visualdictionary masked vision modeling task. E2E-VLP (Xu et al.
2021) presents a pretraining framework supervised with additional object detection and image captioning tasks to enhance visual semantics learning. It is worth noting that their
object detection pretext task requires millions of bounding
boxes annotation, unable to generalize to large-scale imagetext corpus. ViLT (Kim, Son, and Kim 2021) is the first to
unify vision and language with a pure Transformer network,
which has a simpler structure and enjoys faster inference.
However, compared to the two-step methods, they are typically less expressive in terms of object-level concepts and
thus suffer from weaker performances on challenging visual
reasoning tasks. Our method is in line with the E2E pretraining framework. The key difference is that we propose to
facilitate learning object-aware multi-modal representations
by performing object semantic knowledge distillation.

% ------------ end -------------------



















\magenta{``on similar cross-modality pre-training directions:
ViLBERT (Lu et al., 2019) and Visual-BERT (Li et al., 2019). Our LXMERT methods differs from them in multiple ways: we use a more detailed, multi-component design for the crossmodality model (i.e., with an object-relationship encoder and cross-modality layers) and we employ additional, useful pre-training tasks (i.e., RoIfeature regression and image question answering).''} \cite{tan2019lxmert}


% ------------------------------------



\blue{Important!}
ViLT: Vision-and-Language Transformer Without Convolution or Region Supervision \cite{kim2021vilt}
\magenta{``ViLT is the first VLP model of which the modal-specific components require less computation than the transformer component for multimodal interactions.''}

\magenta{``ViLT (Kim, Son, and Kim 2021) is the first to
unify vision and language with a pure Transformer network,
which has a simpler structure and enjoys faster inference.
However, compared to the two-step methods, they are typically less expressive in terms of object-level concepts and
thus suffer from weaker performances on challenging visual
reasoning tasks.'' \cite{liu2021kd}}


% -------------------------------------
\keypoint{Discussion:} addition to the pretext loss functions, other more fine-grained loss iterms can be used to achieve better fusion or alignment, for example, Contrastive loss \cite{zhan2021product1m}. use other matric learning technique, \eg, triplet ranking?


% ----------------------------------

\magenta{``Audio-visual learning. Audio-visual data offers a variety
of resources for knowledge transfer between different modalities [4, 7, 1]. Many works [64, 3] leverage the natural
synchronization between vision and sound to learn representation of sounds and images without ground truth labels.
This has been successfully used in various tasks such as''} \cite{vasudevan2022sound}

% ----------------------------------

PRETEXT TASK -- visual coordinate prediction, spatial skewness prediction, QAs with Grounding, ??? \cite{yun2021pano}


% -----------------------------


VARIANTS \keypoint{\red{some variants of self-attention}}, give some examples:
AoANet, Attention on Attention for Image Captioning, ICCV 2019, citation 290+ \cite{huang2019attention},


% ---------------------------

vision models,

not multi-modal, 

Vision Models Are More Robust And Fair When Pretrained On Uncurated Images Without Supervision \cite{goyal2022vision}

% ------------------------------------

TOPIC: \magenta{``Multiple SSL tasks
(Multi-SSL) that generalizes well for all downstream tasks'' \cite{vasudevan2022sound}}


% -------------------------
"Video Transformers: A Survey"
\red{how to improve/optimize: small query, sparse Sparse approaches, weight sharing, }

% --------------------------


IJCV survey -- Perspectives and Prospects on Transformer Architecture for
Cross-Modal Tasks with Language and Vision

https://link.springer.com/content/pdf/10.1007/s11263-021-01547-8.pdf
